Non-Normal Super-Strict Implications

This paper introduces the logics of super-strict implications that are based on C.I. Lewis' non-normal modal logics S2 and S3. The semantics of these logics is based on Kripke's semantics for non-normal modal logics. This solves a question we left open in a previous paper by showing that these logics are weakly connexive.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{A. Indrzejczak, M. Zawidzki (Eds): 10th International Conference\\on Non-Classical Logics. Theory and Applications (NCL 2022)\\
EPTCS 358, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.358.1}{10.4204/EPTCS.358.1}}

